Video Anomaly Detection and Explanation via Large Language Models

Video Anomaly Detection (VAD) aims to localize abnormal events on the timeline of long-range surveillance videos. Anomaly-scoring-based methods have been prevailing for years but suffer from the high complexity of thresholding and low explanability of detection results. In this paper, we conduct pioneer research on equipping video-based large language models (VLLMs) in the framework of VAD, making the VAD model free from thresholds and able to explain the reasons for the detected anomalies. We introduce a novel network module Long-Term Context (LTC) to mitigate the incapability of VLLMs in long-range context modeling. We design a three-phase training method to improve the efficiency of fine-tuning VLLMs by substantially minimizing the requirements for VAD data and lowering the costs of annotating instruction-tuning data. Our trained model achieves the top performance on the anomaly videos of the UCF-Crime and TAD benchmarks, with the AUC improvements of +3.86\% and +4.96\%, respectively. More impressively, our approach can provide textual explanations for detected anomalies.

==> Sections/Acknowledge.tex <==
\section{Acknowledgments}
The author gratefully acknowledges the support of Alibaba-NTU Singapore Joint Research Institute, the A*STAR under its AME YIRG Grant (Project No.A20E6c0101), the Lee Kong Chian (LKC) Fellowship fund awarded by Singapore Management University, AI Singapore AISG2-RP-2021-022, the Postgraduate Research \& Practice Innovation Program of Jiangsu Province, the National Natural Science Foundation of China (Grants No.62072244), the Natural Science Foundation of Shandong Province (Grant No.ZR2020LZH008) and State Key Laboratory of High-end Server \& Storage Technology.
%This work was also supported in part by State Key Laboratory of High-end Server \& Storage Technology.
